Dynamic Programming for One-Sided Partially Observable Pursuit-Evasion Games

Pursuit-evasion scenarios appear widely in robotics, security domains, and many other real-world situations. We focus on two-player pursuit-evasion games with concurrent moves, infinite horizon, and discounted rewards. We assume that the players have a partial observability, however, the evader is given an advantage of knowing the current position of the units of the pursuer. This setting is particularly interesting for security domains where a robust strategy, designed to maximize the utility in the worst-case scenario, is often desirable. We provide, to the best of our knowledge, the first algorithm that provably converges to the value of a partially observable pursuit-evasion game with infinite horizon. Our algorithm extends well-known value iteration algorithm by exploiting that (1) the value functions of our game depend only on position of the pursuer and the belief he has about the current position of the evader, and (2) that these functions are piecewise linear and convex in the belief space.

==> background.tex <==
We use the notion of finite-horizon POSGs, or \emph{extensive-form games} (EFGs), to reason about the infinite-horizon pursuit-evasion game with discounted reward.
An extensive-form game (EFG) with horizon $T$ is a tuple $G^T=(\calN,\calH,\calZ,\calT,u,{\cal I})$.
$\calN = \{1, 2\}$ is a set of players, by $i$ we refer to one of the players, and by $-i$ to her opponent. 
$\calH$ denotes a finite set of \emph{histories} of actions taken by all players from the root of the game. 
Each history corresponds to a \emph{node} in the game tree; hence, we use the terms history and node interchangeably.
We say that $h$ is a \emph{prefix} of~$h'$ ($h \sqsubseteq h'$) if $h$ lies on a path from the root of the game tree to $h'$.
$\calZ \subseteq \calH$  is the set of all \emph{terminal states} of the game. 
$\calT$ is a transition function that provides a set of actions, or accessible states from a given state.
An ordered list of all transitions of player~$i$ from root to node $h$ is referred to as a \emph{sequence}. 
Each sequence consists of at most $T$ transitions.
%Finally, playing action $a$ in node $h$ leads to node (history) $ha$.
For each $z \in \calZ$ we define a \emph{utility function} $u_i : \calZ \rightarrow \mathbb{R}$ for each player~$i$ ($u_i(z) = -u_{-i}(z)$ in zero-sum games). 
Imperfect observation of player $i$ is modeled via \emph{information sets} ${\cal I}_i$ that form a partition over $h \in \calH$ where $i$ takes action.
Player $i$ cannot distinguish between nodes in any $I_i \in \calI_i$.

